Analyzing rotational bands in odd-mass nuclei using Effective Field Theory and Bayesian methods

We recently developed an Effective Field Theory (EFT) for rotational bands in odd-mass nuclei. Here we use EFT expressions to perform a Bayesian analysis of data on the rotational energy levels of $^{99}$Tc, ${}^{155,157}$Gd, ${}^{159}$Dy, ${}^{167, 169}$Er, ${}^{167, 169}$Tm, ${}^{183}$W, ${}^{235}$U and ${}^{239}$Pu. The error model in our Bayesian analysis includes both experimental and EFT truncation uncertainties. It also accounts for the fact that low-energy constants (LECs) at even and odd orders are expected to have different sizes. We use Markov Chain Monte Carlo (MCMC) sampling to explore the joint posterior of the EFT and error-model parameters and show both the LECs and the expansion parameter, $Q$, can be reliably determined. We extract the LECs up to fourth order in the EFT and find that, provided we correctly account for EFT truncation errors in our likelihood, results for lower-order LECs are stable as we go to higher orders. LEC results are also stable with respect to the addition of higher-energy data. We extract the expansion parameter for all the nuclei listed above and find a clear correlation between the extracted and the expected $Q$ based on the single-particle and vibrational energy scales. However, the $Q$ that actually determines the convergence of the EFT expansion is markedly smaller than would be naively expected based on those scales.

==> Bayesian Rotational Bands-3/buqeye_macros.tex <==
% !TEX root = EMN_Correlations_Analysis.tex

% Define \newsubcommand:
% look whether the following character is _ and, if so, it will merge the subscripts.
\makeatletter
\newcommand\newsubcommand[3]{\newcommand#1{#2\sc@sub{#3}}}
\def\sc@sub#1{\def\sc@thesub{#1}\@ifnextchar_{\sc@mergesubs}{_{\sc@thesub}}}
\def\sc@mergesubs_#1{_{\sc@thesub#1}}

\newcommand\newsupcommand[3]{\newcommand#1{#2\sc@sup{#3}}}
\def\sc@sup#1{\def\sc@thesup{#1}\@ifnextchar^{\sc@mergesups}{^{\sc@thesup}}}
\def\sc@mergesups^#1{^{\sc@thesup#1}}
\makeatother

% Bold version of mathcal
\DeclareMathAlphabet{\mathbcal}{OMS}{cmsy}{b}{n}

% Put in repeated equation to reuse equation number with a prime (Phys Rev style guide)
\newcommand{\eqrevisited}[1]{\tag{\ref*{#1}$^\prime$}}


\newcommand{\calO}{\mathcal{O}}

% Stats
\DeclareMathOperator{\MVT}{MVT}
\DeclareMathOperator{\NIG}{NIG}  % Normal inverse gamma
\DeclareMathOperator{\IG}{IG}  % Inverse gamma
\DeclareMathOperator{\ninvchisq}{N\chi^{--2}}  % Normal Inverse chi2
\DeclareMathOperator{\invchisq}{\chi^{--2}}  % Inverse chi2
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\kernel}{\kappa}
\newcommand{\onevec}{\boldvec{1}}
\newcommand{\identity}{\mathds{I}}
\newcommand{\cbar}{\bar c}
\newcommand{\sdth}{\cbar}
\newcommand{\sdexp}{\sigma}
\newcommand{\sdnugget}{\sigma_n}
\def\addcite#1{\textbf{\color{red}CITE[#1]}}

% \newcommand{\test}[1]{#1^\star}
% \newcommand{\testt}[1]{#1^{\star\star}}
\newcommand{\test}[1]{#1_\star}
\newcommand{\testt}[1]{#1_{\star\star}}

\newcommand{\diagnostic}{\textup{D}}
\DeclareMathOperator{\CI}{CI}
\newcommand{\DCI}{\diagnostic_{\CI}}
\newcommand{\MD}{\textup{MD}}
\newcommand{\DMD}{\diagnostic_{\MD}}
\newcommand{\DVAR}[1]{\inputvec{D}_{\textup{#1}}}
\newcommand{\DVARIT}[1]{\inputvec{D}_{#1}}

\newcommand{\entryc}[1]{\multicolumn{1}{c}{#1}}

\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\Diid}{\diagnostic_{\iid}}
\newcommand{\Dv}{\diagnostic_{\rm v}}

\newcommand{\indicator}{\mathbf{1}}

% NIG prior hyperparameters
\newcommand{\hypm}{\eta}
% \newcommand{\hypv}{v}
% \newcommand{\hypa}{a}
% \newcommand{\hypb}{b}
\newcommand{\hypdisp}{V}
\newcommand{\hypdf}{\nu}
\newcommand{\hyptau}{\tau}

\newcommand{\basisfunc}{b}
\newcommand{\basis}{B}

% \newcommand{\genobstrain}{\genobsset_{\textup{train}}}
% \newcommand{\genobsvalid}{\genobsset_{\textup{val}}}
\newcommand{\ftrain}{\inputvec{f}_{\textup{train}}}
\newcommand{\fvalid}{\inputvec{f}_{\textup{val}}}

\newcommand{\genobsmean}[1]{m_{#1}}
\newcommand{\genobscorr}[1]{R_{#1}}
\newcommand{\genobsbasisfunc}[1]{\basisfunc_{#1}}
\newcommand{\genobsbasisfunctrans}[1]{\basisfunc_{#1}}  % ^\trans
\newcommand{\tildegenobsbasisfunc}[1]{\tilde\basisfunc_{#1}}
\newcommand{\genobsbasis}[1]{\basis_{#1}}

\newcommand{\tildegenobsmean}[1]{\tilde m_{#1}}
\newcommand{\tildegenobscorr}[1]{\tilde R_{#1}}

\newcommand{\discrmean}[1]{m_{\delta #1}}
\newcommand{\discrcorr}[1]{R_{\delta #1}}
\newcommand{\discrbasisfunc}[1]{\basisfunc_{\delta #1}}
\newcommand{\discrbasisfunctrans}[1]{\basisfunc_{\delta #1}}  % ^\trans
\newcommand{\discrbasis}[1]{\basis_{\delta #1}}
\newcommand{\tildediscrbasisfunc}[1]{\tilde\basisfunc_{\delta #1}}

\newcommand{\tildediscrmean}[1]{\tilde m_{\delta #1}}
\newcommand{\tildediscrcorr}[1]{\tilde R_{\delta #1}}


% Prior hyperparameters
\newcommand{\hypprior}[1]{#1_0}
% Conditional parameters
% \newcommand{\cond}[1]{{#1}_\star}
\newcommand{\cond}[1]{#1}


% general definitions
% \newcommand{\beq}{\begin{equation}}
% \newcommand{\eeq}{\end{equation}}

% \newcommand{\bseq}{\begin{subequations}}
% \newcommand{\eseq}{\end{subequations}}

% \newcommand{\ts}{\textstyle}
% \newcommand{\ds}{\displaystyle}
% \newcommand{\wt}{\widetilde}


\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\Msol}{\,\text{M}_{\odot}\xspace}
\newcommand{\Abinitio}{\textit{Ab~initio}\xspace}
\newcommand{\abinitio}{\textit{ab~initio}\xspace}

\newcommand{\fm}{\, \text{fm}}
\newcommand{\fmi}{\, \text{fm}^{-1}}
\newcommand{\fmis}{\, \text{fm}^{-2}}
\newcommand{\fmiq}{\, \text{fm}^{-3}}
\newcommand{\keV}{\, \text{keV}}
\newcommand{\MeV}{\, \text{MeV}}
% \newcommand{\eft}{$\chi$EFT\xspace}

% \newcommand{\la}{\langle}
% \newcommand{\ra}{\rangle}
% \newcommand{\bu}{$\bullet$\ }
% \newcommand{\adag}{a^\dagger}

%\newcommand{\NNLO}{N$^2$LO}
%\newcommand{\NNNLO}{N$^3$LO}
\newcommand{\NLO}{\ensuremath{{\rm NLO}}\xspace}
\newcommand{\NNLO}{\ensuremath{{\rm N}{}^2{\rm LO}}\xspace}
\newcommand{\NNNLO}{\ensuremath{{\rm N}{}^3{\rm LO}}\xspace}
\newcommand{\NNNNLO}{\ensuremath{{\rm N}{}^4{\rm LO}}\xspace}
\newcommand{\NNNNLOp}{\ensuremath{{\rm N}{}^4{\rm LO}+}\xspace}
\newcommand{\NkLO}[1]{\ensuremath{\mathrm{N}^{#1}\mathrm{LO}}\xspace}


\newcommand{\nc}{n_c}
\newcommand{\nlecs}{n_a}
\newcommand{\neff}{\ensuremath{N_{\text{eff}}}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\hyperparam}{\boldsymbol{\theta}}
\newcommand{\param}{\boldsymbol{\theta}}
\newcommand{\len}{\ell}
\newcommand{\lenvec}{\boldsymbol{\ell}}
\newcommand{\lenset}{\ensuremath{L}}
\newcommand{\lenvecset}{\ensuremath{\mathbf{L}}}
\DeclareMathOperator{\GP}{\mathcal{GP}}
\DeclareMathOperator{\TP}{\mathcal{TP}}

% Neutron-proton and nucleon-nucleon
\newcommand{\npr}{\ensuremath{np}}
\newcommand{\NN}{\ensuremath{NN}}

\newcommand{\boldvec}[1]{\bm{#1}}
%\newcommand{\boldvec}[1]{\mathbf{#1}}

\newcommand{\ordervec}{\vec}
\newcommand{\inputdimvec}{}
\newcommand{\inputvec}{\mathbf}
\newcommand{\func}{f}
\newcommand{\funcvec}{\inputvec{\func}}
\newcommand{\meanvec}{\inputvec{m}}

\newcommand{\muth}{m_{\textup{th}}}
\newcommand{\muthset}{\mathbf{m}_{\textup{th}}}
\newcommand{\covth}{\Sigma_{\textup{th}}}
\newcommand{\covexp}{\Sigma_{\textup{exp}}}
% \newcommand{\sdexp}{\sigma_{\textup{exp}}}

% infinite matter
\newcommand{\dens}{\rho}

\newcommand{\betavec}{{\boldsymbol{\beta}}}
% \newcommand{\muvec}{\boldsymbol{\mu}}
\newcommand{\avec}{\boldvec{a}}
\newcommand{\bvec}{\boldvec{b}}
\newcommand{\cvec}{\boldvec{c}}
\newcommand{\evec}{\boldvec{e}}
\newcommand{\nvec}{\boldvec{n}}
\newcommand{\pvec}{\boldvec{p}}
\newcommand{\qvec}{\boldvec{q}}
\newcommand{\vvec}{\boldvec{v}}
\newcommand{\xvec}{\boldvec{x}}
\newcommand{\xvecd}{\boldvec{x'}} % add by myself
\newcommand{\rvec}{\boldvec{r}}
\newcommand{\Rvec}{\boldvec{R}}
\newcommand{\svec}{\boldvec{s}}
\newcommand{\yvec}{\boldvec{y}}
\newcommand{\zvec}{\boldvec{z}}
\newcommand{\muvec}{\boldvec{\mu}}
\newcommand{\sigmavec}[1]{\boldsymbol{\sigma}^{(#1)}}
\newcommand{\ellvec}{\boldvec{\ell}}
\newcommand{\mvec}{\boldvec{m}}
\newcommand{\kvec}{\boldvec{k}}
\newcommand{\kpvec}{\boldvec{k}'}
\newcommand{\kprvec}{\boldvec{k}_{R_1}'}
\newcommand{\spvec}{\boldvec{s}'}
\newcommand{\sprvec}{\boldvec{s}_{R_1}'}
\newcommand{\kppvec}{\boldvec{k}''}
\newcommand{\kpprvec}{\boldvec{k}_{R_2}''}
\newcommand{\sppvec}{\boldvec{s}''}
\newcommand{\spprvec}{\boldvec{s}_{R_2}''}
\newsubcommand{\ckvec}{\ordervec{c}}{k}
\newcommand{\ckvecsq}{\ckvec^{\,2}}

\newsubcommand{\bkvec}{\ordervec{b}}{k}
% \newcommand{\bkvecsq}{\mathbf{b}_k^{2}}
% \newcommand{\kinparvec}{\boldvec{\alpha}}
\newcommand{\kinparvec}{\inputdimvec{x}}
\newcommand{\kinparvecset}{\inputdimvec{\inputvec{x}}}



\newcommand{\kinparvecmag}{x}
% \newsubcommand{\ckvecset}{\mathbf{C}}{k}
\newsubcommand{\ckvecset}{\ordervec{\inputvec{c}}}{k}
% \newcommand{\cbarset}{\bar{C}}
\newcommand{\cset}{C}
\newcommand{\capprox}{\ensuremath{c'}}
\newcommand{\capproxxset}{\ensuremath{C'}}
\newsubcommand{\ckvecapprox}{\mathbf{c}'}{k}
\newsubcommand{\ckvecapproxset}{\mathbf{C}'}{k}
\newcommand{\bset}{B}
\newcommand{\bapprox}{\ensuremath{b'}}
\newcommand{\bapproxset}{\ensuremath{B'}}
\newsubcommand{\bkvecapprox}{\mathbf{b}'}{k}
\newsubcommand{\bkvecset}{\mathbf{B}}{k}
\newsubcommand{\bkvecapproxset}{\mathbf{B}'}{k}


\newcommand{\genobs}{y}
\newcommand{\genobsinput}{\inputdimvec{\genobs}}
\newsubcommand{\genobsvec}{\ordervec{\genobs}}{k}
\newsubcommand{\genobsvecset}{\ordervec{\inputvec{\genobs}}}{k}
\newcommand{\genobsset}{\inputvec{\genobs}}

\newcommand{\genobsexp}{\genobs_{\textup{exp}}}        % subscript or superscript?
\newcommand{\genobsexpset}{\inputvec{\genobs}_{\textup{exp}}}
% \newcommand{\genobsvecexp}{\genobsvec_{\textup{exp}}}    % {\genobsvec^{\mathrm{exp}}}  % subscript or superscript?
\newcommand{\genobsth}{\genobs_{\textup{th}}}          % subscript or superscript?
\newcommand{\genobsthset}{\inputvec{\genobs}_{\textup{th}}}


\newcommand{\qsumm}{q}
\newcommand{\qsumv}{\hat q}

\newcommand{\kord}{k}
\newcommand{\Nexp}{N_d}
\newcommand{\Qvec}{\inputvec{Q}}  % vector of expansion parameters at kinematic points

\newcommand{\lecs}{\vec{a}}
\newcommand{\LEC}{\lecs}
\newcommand{\LECk}{\LEC_k}


\newcommand{\crms}{c_{\mathrm{rms}}}  % empirical estimate of \cbar
\newcommand{\sigmaexp}{\sigma}
\newcommand{\sigmaexpvec}{\inputvec{\sigma}}
\newcommand{\covarexp}{{\Sigma}_{\mathrm{exp}}} % removed \myvec before {\Sigma}   % covariance matrix for experimental errors
\newcommand{\covarth}{{\Sigma}_{\mathrm{th}}}  % removed \myvec before {\Sigma}   % covariance matrix for theory errors
\newcommand{\covarLEC}{{\Sigma}_{\mathrm{LECs}}}
\newcommand{\covartrunc}{{\Sigma}_{k}}


\newsubcommand{\akvec}{\mathbf{a}}{k}
\newcommand{\aset}{A}
\newcommand{\aapprox}{\ensuremath{a'}}
\newcommand{\aapproxset}{\ensuremath{A'}}
\newsubcommand{\akvecapprox}{\mathbf{a}'}{k}
\newsubcommand{\akvecset}{\mathbf{A}}{k}
\newsubcommand{\akvecapproxset}{\mathbf{A}'}{k}


% \newcommand{\bi}{\begin{itemize}}
% \newcommand{\ei}{\end{itemize}}
% \newcommand{\I}{\item}
% \newcommand{\be}{\begin{enumerate}}
% \newcommand{\ee}{\end{enumerate}}
% \newcommand{\bc}{\begin{center}}
% \newcommand{\ec}{\end{center}}


\newcommand{\Covfunc}{\ensuremath{k}}
\newcommand{\Covmat}{\vb{K}}
\newcommand{\Corrmat}{\vb{R}}
\newcommand{\Covmattest}{\boldsymbol{\Sigma}}


%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%
% The \pr command
%%%%%%%%%%%%%%%%%%%

\let\Pr\undefined{}  % Remove the definition from the Physics package

% \newcommand{\pr}{\text{pr}} % Old
\DeclareMathOperator{\pr}{pr} % Good, but want to handle sizing and | spacing?
% \DeclareDocumentCommand\pr{}{\opbraces{\prob}} % Using opbraces from physics package to resize delimeters
\newcommand{\given}{\,|\,}  % Use for | in \pr
\DeclareMathOperator{\prior}{\pi}

% From https://tex.stackexchange.com/questions/187162/vertical-bar-for-absolute-value-and-conditional-expectation
% Can use automatic resizing with * or manual with [\Big] etc.
% Also can edit the spacing that | provides via innermid
% \newcommand{\prob}{\operatorname{pr}\expectarg}
% \DeclarePairedDelimiterX{\expectarg}[1]{(}{)}{%
%   \ifnum\currentgrouptype=16 \else\begingroup\fi
%   \activatebar#1
%   \ifnum\currentgrouptype=16 \else\endgroup\fi
% }

% \newcommand{\innermid}{\nonscript\;\delimsize\vert\nonscript\;}
% \newcommand{\activatebar}{%
%   \begingroup\lccode`\~=`\|
%   \lowercase{\endgroup\let~}\innermid 
%   \mathcode`|=\string"8000
% }

%%%%%%%%%%%%%%%%%%%%%%%%






% \newcommand{\cmarg}{\mathbf{c}_{\text{marg}}}
% \newcommand{\amarg}{\mathbf{a}_{\text{marg}}}
% \newcommand{\Amat}{\widehat{A}}
% \newcommand{\ares}{\mathbf{a}_{\text{res}}}
% %newcommand{\amarg}{\mathbf{a}_{\text{marg}}}
% \newcommand{\dif}{\mathrm{d}}
% \newcommand{\alphavec}{\boldsymbol{\alpha}}
% \newcommand{\fvec}{\boldsymbol{f}}
% \newcommand{\Dvec}{\boldsymbol{D}}
% \newcommand{\Covmat}{\widehat{\boldsymbol{\Sigma}}}
% \newcommand{\Modeltxt}{$\mathcal{M}\,\,$}
% \newcommand{\ED}{\mathcal{H}}
% \newcommand{\Model}{\mathcal{M}}
% \newcommand{\lhood}{\mathcal{L}}
% \newcommand{\gth}{g_{\text{th}}}
% \newcommand{\gthtwo}{g_{\text{th},2}}
% \newcommand{\hth}{h_{\text{th}}}
% \newcommand{\MchiPT}{M_{\chi \text{PT}}}
% \newcommand{\ktilde}{\tilde{k}}
% \newcommand{\Mtilde}{\widetilde{M}}
% \newcommand{\loglammu}{\log \left( \frac{\Lambda}{\mu} \right)}
% \newcommand{\mmax}{m_{max}}
% \newcommand{\fth}{f_{\text{th}}}
% \newcommand{\xmax}{x_{\text{max}}}
\newcommand{\kmax}{k_{\text{max}}}
\newcommand{\abar}{\bar{a}}
% \newcommand{\abarfix}{\abar_{\rm fix}}

%\newcommand{\cbar}{\overline{c}}
% \newcommand{\cbar}{\bar{c}}
% \newcommand{\cbarsubk}[1]{\cbar_{(#1)}}
% \newcommand{\cbark}{\cbarsubk{k}}
% \newcommand{\cbarmin}{\cbar_{<}}
% \newcommand{\cbarmax}{\cbar_{>}}

\newcommand{\lbar}{\bar{l}}
\newcommand{\Rmat}{\widehat{R}}

\newcommand{\Q}{\ensuremath{Q}}
\newcommand{\Qapprox}{\ensuremath{Q'}}
\newcommand{\Qmax}{\Q_{\rm max}}
\newcommand{\smallscale}{\ensuremath{\mathcal{Q}}}
\newcommand{\smallscaleapprox}{\ensuremath{\mathcal{Q}'}}

\newcommand{\Elab}{E_{\rm lab}}
\newcommand{\krel}{k_{\rm rel}}
\newcommand{\prel}{p_{\rm rel}}
\newcommand{\qrel}{q_{\rm rel}}
\newcommand{\kzero}{k_0}
\newcommand{\degr}{\circ}

\newcommand{\signp}{\sigma_{np}}

\newcommand{\normal}{\mathcal{N}}

% \newcommand{\atan}{\arctan}
% \newcommand{\asin}{\arcsin}


% \newcommand{\pdf}{\pr}  % {f}   % adjust this as desired.  E.g., f --> \pr
% \newcommand{\feps}{\pdf_{\epsilon}}
% \newcommand{\CH}{CH}
% \newcommand{\CHbar}{$\overline{\rm CH}$}
% \newcommand{\aSbar}{\bar{\alpha}_S}


\newcommand{\NNLOsim}{NNLO$_\text{sim}$}
\newcommand{\NNLOsep}{NNLO$_\text{sep}$}
\newcommand{\NNLOsat}{\ensuremath{\mathrm{NNLO}_{\mathrm{sat}}}}
\newcommand{\Info}{\mathcal{H}}
\newcommand{\dobs}{\tilde{d}}
\newcommand{\Htilde}{\tilde{H}}
\newcommand{\ModelT}{\text{T}}

\newcommand{\Aaug}{\matr{A}_{\textrm{aug}}}
\newcommand{\thetavec}{\bm{\theta}}
\newcommand{\dataset}[3]{\ensuremath{{\textrm #1}#2_{(#3\%)}}}
%\newcommand{\kmax}{k_{\text{max}}}

\newcommand{\Cprime}{C$'$}

% notation for matrices
%\newcommand{\matr}[1]{\mathbf{#1}} % undergraduate algebra version
\newcommand{\matr}[1]{#1}          % pure math version
%\newcommand{\matr}[1]{\bm{#1}}     % ISO complying version

\newcommand{\transpose}[1]{{#1}^{\intercal}}
\newcommand{\trans}{\intercal}


\newcommand{\ktrue}{k^{\rm true}}
\newcommand{\atrue}{a^{\rm true}}
\newcommand{\avecmin}{\hat\avec}
\newcommand{\Nd}{N_d}

\newcommand{\chiEFT}{$\chi$EFT}
\newcommand{\chisq}{\chi^2}
\newcommand{\chisqaug}{\chisq_{\textrm aug}}
\newcommand{\avecaug}{\avec_{\textrm aug}}

\newcommand{\CHtoEKM}{CH\_to\_EKM}
\newcommand{\LamchiSB}{\Lambda_{\chi {\rm SB}}}
\newcommand{\chiPT}{\chi{\rm PT}}

% \newcommand{\Data}{\ensuremath{c_0,\ldots,c_k}}
\newcommand{\Aeps}{\ensuremath{{\rm A}_{\epsilon}}}
\newcommand{\Ceps}{\ensuremath{{\rm C}_{\epsilon}}}
\newcommand{\Aepsone}{\Aeps^{(1)}}
\newcommand{\Cepsone}{\Ceps^{(1)}}
\newcommand{\Aone}{\ensuremath{{\rm A}^{(1)}}}
\newcommand{\Bone}{\ensuremath{{\rm B}^{(1)}}}
\newcommand{\Cone}{\ensuremath{{\rm C}^{(1)}}}
\newcommand{\Af}[2]{\ensuremath{{\rm A}_{#1\text{-}#2}}}
\newcommand{\Cf}[2]{\ensuremath{{\rm C}_{#1\text{-}#2}}}
\newcommand{\Afone}[2]{\Af{#1}{#2}^{(1)}}
\newcommand{\Cfone}[2]{\Cf{#1}{#2}^{(1)}}
\newcommand{\Deltakone}{\ensuremath{\Delta_k^{(1)}}}
\newcommand{\dkp}{\ensuremath{d_k^{(p)}}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\sbarmin}{\sbar_{<}}
\newcommand{\sbarmax}{\sbar_{>}}
\newcommand{\ppercentt}{\ensuremath{\left(p\%\right)_{\rm t}}}

% \newcommand{\Xref}{\ensuremath{\mathcal{X}_{\text{ref}}}}
% \newcommand{\Xrefinput}{\ensuremath{\mathbcal{X}_{\text{ref}}}}
\newcommand{\genobsref}{\ensuremath{y_{\mathrm{ref}}}}
\newcommand{\genobsrefset}{\ensuremath{\inputvec{y}_{\mathrm{ref}}}}
\newcommand{\genobsrefinput}{\ensuremath{\inputdimvec{y}_{\mathrm{ref}}}}

\newcommand{\Mmatrix}[3]{M^{#1}_{{#2}\,{#3}}}
\newcommand{\CG}[6]{\langle {#1}\,{#2}\; {#3}\,{#4} | {#5}\,{#6} \rangle}
\newcommand{\sigmatot}{\sigma_{\text{tot}}}
\newcommand{\sigmaref}{\sigma_{\text {ref}}}
\newcommand{\epsbar}{\bar\varepsilon}


\newcommand{\ppercent}{(100*p)\%}

% Glockle Coefficients
\newcommand{\aG}{\ensuremath a_G}
\newcommand{\bG}{\ensuremath b_G}
\newcommand{\cG}{\ensuremath c_G}
\newcommand{\mG}{\ensuremath m_G}
\newcommand{\gG}{\ensuremath g_G}
\newcommand{\hG}{\ensuremath h_G}

% Phase notation
\newcommand{\phase}[3]{\ensuremath{\bar\delta^{#1 #3}_{#2}}}
\newcommand{\blattphase}[3]{\ensuremath{\delta^{#1 #3}_{#2}}}
\newcommand{\epsmix}[1]{\ensuremath{\bar\epsilon_{#1}}}
\newcommand{\blattepsmix}[1]{\ensuremath{\epsilon_{#1}}}
\newcommand{\gammix}[1]{\ensuremath{\bar\gamma_{#1}}}

% R on-shell
\newcommand{\Ron}[4]{R^{#1 #4}_{#2 #3}}


% Lab system / center of momentum system
\newcommand{\ls}{l.s.}
\newcommand{\cms}{c.m.}

\newcommand{\kf}{\ensuremath{k_{\scriptscriptstyle\textrm{F}}}}
\newcommand{\kfzero}{\ensuremath{k_{\scriptscriptstyle\textrm{F,0}}}}

\newcommand{\NEVC}{\ensuremath{N_{\rm EVC}}}


% Differential taken from Physics package
% Uses smart spacing for a nice look. Requires xparse.
% https://www.ctan.org/pkg/physics?lang=en

% First, the basics:
\def\diffd{\mathrm{d}}  % Upright differentials
% \def\diffd{d}  % Italic differentials

% Now add spacing:
% Derivatives
\DeclareDocumentCommand\differential{ o g d() }{ % Differential 'd'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
            {\diffd\IfNoValueTF{#1}{}{^{#1}}}
            {\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
        }
        {\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
    }
\DeclareDocumentCommand\dd{}{\differential} % Shorthand for \differential


% Path Derivative:
\newcommand{\pathd}{\mathcal{D}}  % differential symbol for path integrals

% Now add relevant spacing and options
% Inspired by differential definition from `Physics' package at
% https://www.ctan.org/tex-archive/macros/latex/contrib/physics?lang=en
\DeclareDocumentCommand\pathdifferential{ o g d() }{ % Path 'D'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
            {\pathd\IfNoValueTF{#1}{}{^{#1}}}
            {\mathinner{\pathd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
        }
        {\mathinner{\pathd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
    }

\DeclareDocumentCommand\DD{}{\pathdifferential} % Shorthand for \pathdifferential

% Observable notation

% \newcommand{\dsigma}{\ensuremath{\frac{\partial\sigma}{\partial\Omega}}}

% \makeatletter
% \def\dsigma{\@ifstar\@@dsigmawithstar\@dsigma}
% \def\@dsigma{\frac{\dd\sigma}{\dd\Omega}}  % \dsigma for upright frac
% \def\@@dsigmawithstar{\dd\sigma/\dd\Omega} % \dsigma* for inline frac
% \makeatother

% From physics package. Optimal braces.
% \DeclareDocumentCommand\argopen{s}{\IfBooleanTF{#1}{\mathopen{}\mathclose\bgroup}{\mathopen{}\mathclose\bgroup\left}} % Special open grouping for argument of a function
% \DeclareDocumentCommand\argclose{s}{\IfBooleanTF{#1}{\egroup}{\aftergroup\egroup\right}} % Special close grouping for argument of a function

% \DeclareDocumentCommand\braces{}{{\ifnum\z@=`}\fi\@braces}
% \DeclareDocumentCommand\@braces{ s t\big t\Big t\bigg t\Bigg m m m }
% { % General braces with automatic and manual sizing
%     \IfBooleanTF{#1}
%     {\left#6\smash{#8}\right#7\vphantom{#8}}
%     {
%         \IfBooleanTF{#2}{\bigl#6{#8}\bigr#7}{
%             \IfBooleanTF{#3}{\Bigl#6{#8}\Bigr#7}{
%                 \IfBooleanTF{#4}{\biggl#6{#8}\biggr#7}{
%                     \IfBooleanTF{#5}{\Biggl#6{#8}\Biggr#7}{\left#6{#8}\right#7}
%                 }
%             }
%         }
%     }
%     \ifnum\z@=`{\fi}
% }

% \DeclareDocumentCommand\fbraces{ s t\big t\Big t\bigg t\Bigg m m m m }
% { % Function braces with automatic and manual sizing
%     #8
%     \IfBooleanTF{#1}
%     {\argopen#6\smash{#9}\argclose#7\vphantom{#9}}
%     {
%         \IfBooleanTF{#2}{\argopen*\bigl#6{#9}\argclose*\bigr#7}{
%             \IfBooleanTF{#3}{\argopen*\Bigl#6{#9}\argclose*\Bigr#7}{
%                 \IfBooleanTF{#4}{\argopen*\biggl#6{#9}\argclose*\biggr#7}{
%                     \IfBooleanTF{#5}
%                     {\argopen*\Biggl#6{#9}\argclose*\Biggr#7}
%                     {\argopen#6{#9}\argclose#7}
%                 }
%             }
%         }
%     }
% }
% \DeclareDocumentCommand\opbraces{ m g o d() }
% {
%     \IfNoValueTF{#2}
%     {
%         \IfNoValueTF{#3}
%             {
%                 \IfNoValueTF{#4}
%                 {#1}
%                 {\fbraces{\lparen}{\rparen}{#1}{#4}}
%             }
%             {
%                 \fbraces{\lbrack}{\rbrack}{#1}{#3}
%                 \IfNoValueTF{#4}{}{(#4)}
%             }
%     }
%     {
%         \fbraces{\lbrace}{\rbrace}{#1}{#2}
%         \IfNoValueTF{#3}{}{[#3]}
%         \IfNoValueTF{#4}{}{(#4)}
%     }
% }

% \let\exponential\exp \DeclareDocumentCommand\exp{}{\opbraces{\exponential}}


==> buqeye_macros.tex <==
% !TEX root = EMN_Correlations_Analysis.tex

% Define \newsubcommand:
% look whether the following character is _ and, if so, it will merge the subscripts.
\makeatletter
\newcommand\newsubcommand[3]{\newcommand#1{#2\sc@sub{#3}}}
\def\sc@sub#1{\def\sc@thesub{#1}\@ifnextchar_{\sc@mergesubs}{_{\sc@thesub}}}
\def\sc@mergesubs_#1{_{\sc@thesub#1}}

\newcommand\newsupcommand[3]{\newcommand#1{#2\sc@sup{#3}}}
\def\sc@sup#1{\def\sc@thesup{#1}\@ifnextchar^{\sc@mergesups}{^{\sc@thesup}}}
\def\sc@mergesups^#1{^{\sc@thesup#1}}
\makeatother

% Bold version of mathcal
\DeclareMathAlphabet{\mathbcal}{OMS}{cmsy}{b}{n}

% Put in repeated equation to reuse equation number with a prime (Phys Rev style guide)
\newcommand{\eqrevisited}[1]{\tag{\ref*{#1}$^\prime$}}


\newcommand{\calO}{\mathcal{O}}

% Stats
\DeclareMathOperator{\MVT}{MVT}
\DeclareMathOperator{\NIG}{NIG}  % Normal inverse gamma
\DeclareMathOperator{\IG}{IG}  % Inverse gamma
\DeclareMathOperator{\ninvchisq}{N\chi^{--2}}  % Normal Inverse chi2
\DeclareMathOperator{\invchisq}{\chi^{--2}}  % Inverse chi2
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\kernel}{\kappa}
\newcommand{\onevec}{\boldvec{1}}
\newcommand{\identity}{\mathds{I}}
\newcommand{\cbar}{\bar c}
\newcommand{\sdth}{\cbar}
\newcommand{\sdexp}{\sigma}
\newcommand{\sdnugget}{\sigma_n}
\def\addcite#1{\textbf{\color{red}CITE[#1]}}

% \newcommand{\test}[1]{#1^\star}
% \newcommand{\testt}[1]{#1^{\star\star}}
\newcommand{\test}[1]{#1_\star}
\newcommand{\testt}[1]{#1_{\star\star}}

\newcommand{\diagnostic}{\textup{D}}
\DeclareMathOperator{\CI}{CI}
\newcommand{\DCI}{\diagnostic_{\CI}}
\newcommand{\MD}{\textup{MD}}
\newcommand{\DMD}{\diagnostic_{\MD}}
\newcommand{\DVAR}[1]{\inputvec{D}_{\textup{#1}}}
\newcommand{\DVARIT}[1]{\inputvec{D}_{#1}}

\newcommand{\entryc}[1]{\multicolumn{1}{c}{#1}}

\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\Diid}{\diagnostic_{\iid}}
\newcommand{\Dv}{\diagnostic_{\rm v}}

\newcommand{\indicator}{\mathbf{1}}

% NIG prior hyperparameters
\newcommand{\hypm}{\eta}
% \newcommand{\hypv}{v}
% \newcommand{\hypa}{a}
% \newcommand{\hypb}{b}
\newcommand{\hypdisp}{V}
\newcommand{\hypdf}{\nu}
\newcommand{\hyptau}{\tau}

\newcommand{\basisfunc}{b}
\newcommand{\basis}{B}

% \newcommand{\genobstrain}{\genobsset_{\textup{train}}}
% \newcommand{\genobsvalid}{\genobsset_{\textup{val}}}
\newcommand{\ftrain}{\inputvec{f}_{\textup{train}}}
\newcommand{\fvalid}{\inputvec{f}_{\textup{val}}}

\newcommand{\genobsmean}[1]{m_{#1}}
\newcommand{\genobscorr}[1]{R_{#1}}
\newcommand{\genobsbasisfunc}[1]{\basisfunc_{#1}}
\newcommand{\genobsbasisfunctrans}[1]{\basisfunc_{#1}}  % ^\trans
\newcommand{\tildegenobsbasisfunc}[1]{\tilde\basisfunc_{#1}}
\newcommand{\genobsbasis}[1]{\basis_{#1}}

\newcommand{\tildegenobsmean}[1]{\tilde m_{#1}}
\newcommand{\tildegenobscorr}[1]{\tilde R_{#1}}

\newcommand{\discrmean}[1]{m_{\delta #1}}
\newcommand{\discrcorr}[1]{R_{\delta #1}}
\newcommand{\discrbasisfunc}[1]{\basisfunc_{\delta #1}}
\newcommand{\discrbasisfunctrans}[1]{\basisfunc_{\delta #1}}  % ^\trans
\newcommand{\discrbasis}[1]{\basis_{\delta #1}}
\newcommand{\tildediscrbasisfunc}[1]{\tilde\basisfunc_{\delta #1}}

\newcommand{\tildediscrmean}[1]{\tilde m_{\delta #1}}
\newcommand{\tildediscrcorr}[1]{\tilde R_{\delta #1}}


% Prior hyperparameters
\newcommand{\hypprior}[1]{#1_0}
% Conditional parameters
% \newcommand{\cond}[1]{{#1}_\star}
\newcommand{\cond}[1]{#1}


% general definitions
% \newcommand{\beq}{\begin{equation}}
% \newcommand{\eeq}{\end{equation}}

% \newcommand{\bseq}{\begin{subequations}}
% \newcommand{\eseq}{\end{subequations}}

% \newcommand{\ts}{\textstyle}
% \newcommand{\ds}{\displaystyle}
% \newcommand{\wt}{\widetilde}


\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\Msol}{\,\text{M}_{\odot}\xspace}
\newcommand{\Abinitio}{\textit{Ab~initio}\xspace}
\newcommand{\abinitio}{\textit{ab~initio}\xspace}

\newcommand{\fm}{\, \text{fm}}
\newcommand{\fmi}{\, \text{fm}^{-1}}
\newcommand{\fmis}{\, \text{fm}^{-2}}
\newcommand{\fmiq}{\, \text{fm}^{-3}}
\newcommand{\keV}{\, \text{keV}}
\newcommand{\MeV}{\, \text{MeV}}
% \newcommand{\eft}{$\chi$EFT\xspace}

% \newcommand{\la}{\langle}
% \newcommand{\ra}{\rangle}
% \newcommand{\bu}{$\bullet$\ }
% \newcommand{\adag}{a^\dagger}

%\newcommand{\NNLO}{N$^2$LO}
%\newcommand{\NNNLO}{N$^3$LO}
\newcommand{\NLO}{\ensuremath{{\rm NLO}}\xspace}
\newcommand{\NNLO}{\ensuremath{{\rm N}{}^2{\rm LO}}\xspace}
\newcommand{\NNNLO}{\ensuremath{{\rm N}{}^3{\rm LO}}\xspace}
\newcommand{\NNNNLO}{\ensuremath{{\rm N}{}^4{\rm LO}}\xspace}
\newcommand{\NNNNLOp}{\ensuremath{{\rm N}{}^4{\rm LO}+}\xspace}
\newcommand{\NkLO}[1]{\ensuremath{\mathrm{N}^{#1}\mathrm{LO}}\xspace}


\newcommand{\nc}{n_c}
\newcommand{\nlecs}{n_a}
\newcommand{\neff}{\ensuremath{N_{\text{eff}}}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\hyperparam}{\boldsymbol{\theta}}
\newcommand{\param}{\boldsymbol{\theta}}
\newcommand{\len}{\ell}
\newcommand{\lenvec}{\boldsymbol{\ell}}
\newcommand{\lenset}{\ensuremath{L}}
\newcommand{\lenvecset}{\ensuremath{\mathbf{L}}}
\DeclareMathOperator{\GP}{\mathcal{GP}}
\DeclareMathOperator{\TP}{\mathcal{TP}}

% Neutron-proton and nucleon-nucleon
\newcommand{\npr}{\ensuremath{np}}
\newcommand{\NN}{\ensuremath{NN}}

\newcommand{\boldvec}[1]{\bm{#1}}
%\newcommand{\boldvec}[1]{\mathbf{#1}}

\newcommand{\ordervec}{\vec}
\newcommand{\inputdimvec}{}
\newcommand{\inputvec}{\mathbf}
\newcommand{\func}{f}
\newcommand{\funcvec}{\inputvec{\func}}
\newcommand{\meanvec}{\inputvec{m}}

\newcommand{\muth}{m_{\textup{th}}}
\newcommand{\muthset}{\mathbf{m}_{\textup{th}}}
\newcommand{\covth}{\Sigma_{\textup{th}}}
\newcommand{\covexp}{\Sigma_{\textup{exp}}}
% \newcommand{\sdexp}{\sigma_{\textup{exp}}}

% infinite matter
\newcommand{\dens}{\rho}

\newcommand{\betavec}{{\boldsymbol{\beta}}}
% \newcommand{\muvec}{\boldsymbol{\mu}}
\newcommand{\avec}{\boldvec{a}}
\newcommand{\bvec}{\boldvec{b}}
\newcommand{\cvec}{\boldvec{c}}
\newcommand{\evec}{\boldvec{e}}
\newcommand{\nvec}{\boldvec{n}}
\newcommand{\pvec}{\boldvec{p}}
\newcommand{\qvec}{\boldvec{q}}
\newcommand{\vvec}{\boldvec{v}}
\newcommand{\xvec}{\boldvec{x}}
\newcommand{\xvecd}{\boldvec{x'}} % add by myself
\newcommand{\rvec}{\boldvec{r}}
\newcommand{\Rvec}{\boldvec{R}}
\newcommand{\svec}{\boldvec{s}}
\newcommand{\yvec}{\boldvec{y}}
\newcommand{\zvec}{\boldvec{z}}
\newcommand{\muvec}{\boldvec{\mu}}
\newcommand{\sigmavec}[1]{\boldsymbol{\sigma}^{(#1)}}
\newcommand{\ellvec}{\boldvec{\ell}}
\newcommand{\mvec}{\boldvec{m}}
\newcommand{\kvec}{\boldvec{k}}
\newcommand{\kpvec}{\boldvec{k}'}
\newcommand{\kprvec}{\boldvec{k}_{R_1}'}
\newcommand{\spvec}{\boldvec{s}'}
\newcommand{\sprvec}{\boldvec{s}_{R_1}'}
\newcommand{\kppvec}{\boldvec{k}''}
\newcommand{\kpprvec}{\boldvec{k}_{R_2}''}
\newcommand{\sppvec}{\boldvec{s}''}
\newcommand{\spprvec}{\boldvec{s}_{R_2}''}
\newsubcommand{\ckvec}{\ordervec{c}}{k}
\newcommand{\ckvecsq}{\ckvec^{\,2}}

\newsubcommand{\bkvec}{\ordervec{b}}{k}
% \newcommand{\bkvecsq}{\mathbf{b}_k^{2}}
% \newcommand{\kinparvec}{\boldvec{\alpha}}
\newcommand{\kinparvec}{\inputdimvec{x}}
\newcommand{\kinparvecset}{\inputdimvec{\inputvec{x}}}



\newcommand{\kinparvecmag}{x}
% \newsubcommand{\ckvecset}{\mathbf{C}}{k}
\newsubcommand{\ckvecset}{\ordervec{\inputvec{c}}}{k}
% \newcommand{\cbarset}{\bar{C}}
\newcommand{\cset}{C}
\newcommand{\capprox}{\ensuremath{c'}}
\newcommand{\capproxxset}{\ensuremath{C'}}
\newsubcommand{\ckvecapprox}{\mathbf{c}'}{k}
\newsubcommand{\ckvecapproxset}{\mathbf{C}'}{k}
\newcommand{\bset}{B}
\newcommand{\bapprox}{\ensuremath{b'}}
\newcommand{\bapproxset}{\ensuremath{B'}}
\newsubcommand{\bkvecapprox}{\mathbf{b}'}{k}
\newsubcommand{\bkvecset}{\mathbf{B}}{k}
\newsubcommand{\bkvecapproxset}{\mathbf{B}'}{k}


\newcommand{\genobs}{y}
\newcommand{\genobsinput}{\inputdimvec{\genobs}}
\newsubcommand{\genobsvec}{\ordervec{\genobs}}{k}
\newsubcommand{\genobsvecset}{\ordervec{\inputvec{\genobs}}}{k}
\newcommand{\genobsset}{\inputvec{\genobs}}

\newcommand{\genobsexp}{\genobs_{\textup{exp}}}        % subscript or superscript?
\newcommand{\genobsexpset}{\inputvec{\genobs}_{\textup{exp}}}
% \newcommand{\genobsvecexp}{\genobsvec_{\textup{exp}}}    % {\genobsvec^{\mathrm{exp}}}  % subscript or superscript?
\newcommand{\genobsth}{\genobs_{\textup{th}}}          % subscript or superscript?
\newcommand{\genobsthset}{\inputvec{\genobs}_{\textup{th}}}


\newcommand{\qsumm}{q}
\newcommand{\qsumv}{\hat q}

\newcommand{\kord}{k}
\newcommand{\Nexp}{N_d}
\newcommand{\Qvec}{\inputvec{Q}}  % vector of expansion parameters at kinematic points

\newcommand{\lecs}{\vec{a}}
\newcommand{\LEC}{\lecs}
\newcommand{\LECk}{\LEC_k}


\newcommand{\crms}{c_{\mathrm{rms}}}  % empirical estimate of \cbar
\newcommand{\sigmaexp}{\sigma}
\newcommand{\sigmaexpvec}{\inputvec{\sigma}}
\newcommand{\covarexp}{{\Sigma}_{\mathrm{exp}}} % removed \myvec before {\Sigma}   % covariance matrix for experimental errors
\newcommand{\covarth}{{\Sigma}_{\mathrm{th}}}  % removed \myvec before {\Sigma}   % covariance matrix for theory errors
\newcommand{\covarLEC}{{\Sigma}_{\mathrm{LECs}}}
\newcommand{\covartrunc}{{\Sigma}_{k}}


\newsubcommand{\akvec}{\mathbf{a}}{k}
\newcommand{\aset}{A}
\newcommand{\aapprox}{\ensuremath{a'}}
\newcommand{\aapproxset}{\ensuremath{A'}}
\newsubcommand{\akvecapprox}{\mathbf{a}'}{k}
\newsubcommand{\akvecset}{\mathbf{A}}{k}
\newsubcommand{\akvecapproxset}{\mathbf{A}'}{k}


% \newcommand{\bi}{\begin{itemize}}
% \newcommand{\ei}{\end{itemize}}
% \newcommand{\I}{\item}
% \newcommand{\be}{\begin{enumerate}}
% \newcommand{\ee}{\end{enumerate}}
% \newcommand{\bc}{\begin{center}}
% \newcommand{\ec}{\end{center}}


\newcommand{\Covfunc}{\ensuremath{k}}
\newcommand{\Covmat}{\vb{K}}
\newcommand{\Corrmat}{\vb{R}}
\newcommand{\Covmattest}{\boldsymbol{\Sigma}}


%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%
% The \pr command
%%%%%%%%%%%%%%%%%%%

\let\Pr\undefined{}  % Remove the definition from the Physics package

% \newcommand{\pr}{\text{pr}} % Old
\DeclareMathOperator{\pr}{pr} % Good, but want to handle sizing and | spacing?
% \DeclareDocumentCommand\pr{}{\opbraces{\prob}} % Using opbraces from physics package to resize delimeters
\newcommand{\given}{\,|\,}  % Use for | in \pr
\DeclareMathOperator{\prior}{\pi}

% From https://tex.stackexchange.com/questions/187162/vertical-bar-for-absolute-value-and-conditional-expectation
% Can use automatic resizing with * or manual with [\Big] etc.
% Also can edit the spacing that | provides via innermid
% \newcommand{\prob}{\operatorname{pr}\expectarg}
% \DeclarePairedDelimiterX{\expectarg}[1]{(}{)}{%
%   \ifnum\currentgrouptype=16 \else\begingroup\fi
%   \activatebar#1
%   \ifnum\currentgrouptype=16 \else\endgroup\fi
% }

% \newcommand{\innermid}{\nonscript\;\delimsize\vert\nonscript\;}
% \newcommand{\activatebar}{%
%   \begingroup\lccode`\~=`\|
%   \lowercase{\endgroup\let~}\innermid 
%   \mathcode`|=\string"8000
% }

%%%%%%%%%%%%%%%%%%%%%%%%






% \newcommand{\cmarg}{\mathbf{c}_{\text{marg}}}
% \newcommand{\amarg}{\mathbf{a}_{\text{marg}}}
% \newcommand{\Amat}{\widehat{A}}
% \newcommand{\ares}{\mathbf{a}_{\text{res}}}
% %newcommand{\amarg}{\mathbf{a}_{\text{marg}}}
% \newcommand{\dif}{\mathrm{d}}
% \newcommand{\alphavec}{\boldsymbol{\alpha}}
% \newcommand{\fvec}{\boldsymbol{f}}
% \newcommand{\Dvec}{\boldsymbol{D}}
% \newcommand{\Covmat}{\widehat{\boldsymbol{\Sigma}}}
% \newcommand{\Modeltxt}{$\mathcal{M}\,\,$}
% \newcommand{\ED}{\mathcal{H}}
% \newcommand{\Model}{\mathcal{M}}
% \newcommand{\lhood}{\mathcal{L}}
% \newcommand{\gth}{g_{\text{th}}}
% \newcommand{\gthtwo}{g_{\text{th},2}}
% \newcommand{\hth}{h_{\text{th}}}
% \newcommand{\MchiPT}{M_{\chi \text{PT}}}
% \newcommand{\ktilde}{\tilde{k}}
% \newcommand{\Mtilde}{\widetilde{M}}
% \newcommand{\loglammu}{\log \left( \frac{\Lambda}{\mu} \right)}
% \newcommand{\mmax}{m_{max}}
% \newcommand{\fth}{f_{\text{th}}}
% \newcommand{\xmax}{x_{\text{max}}}
\newcommand{\kmax}{k_{\text{max}}}
\newcommand{\abar}{\bar{a}}
% \newcommand{\abarfix}{\abar_{\rm fix}}

%\newcommand{\cbar}{\overline{c}}
% \newcommand{\cbar}{\bar{c}}
% \newcommand{\cbarsubk}[1]{\cbar_{(#1)}}
% \newcommand{\cbark}{\cbarsubk{k}}
% \newcommand{\cbarmin}{\cbar_{<}}
% \newcommand{\cbarmax}{\cbar_{>}}

\newcommand{\lbar}{\bar{l}}
\newcommand{\Rmat}{\widehat{R}}

\newcommand{\Q}{\ensuremath{Q}}
\newcommand{\Qapprox}{\ensuremath{Q'}}
\newcommand{\Qmax}{\Q_{\rm max}}
\newcommand{\smallscale}{\ensuremath{\mathcal{Q}}}
\newcommand{\smallscaleapprox}{\ensuremath{\mathcal{Q}'}}

\newcommand{\Elab}{E_{\rm lab}}
\newcommand{\krel}{k_{\rm rel}}
\newcommand{\prel}{p_{\rm rel}}
\newcommand{\qrel}{q_{\rm rel}}
\newcommand{\kzero}{k_0}
\newcommand{\degr}{\circ}

\newcommand{\signp}{\sigma_{np}}

\newcommand{\normal}{\mathcal{N}}

% \newcommand{\atan}{\arctan}
% \newcommand{\asin}{\arcsin}


% \newcommand{\pdf}{\pr}  % {f}   % adjust this as desired.  E.g., f --> \pr
% \newcommand{\feps}{\pdf_{\epsilon}}
% \newcommand{\CH}{CH}
% \newcommand{\CHbar}{$\overline{\rm CH}$}
% \newcommand{\aSbar}{\bar{\alpha}_S}


\newcommand{\NNLOsim}{NNLO$_\text{sim}$}
\newcommand{\NNLOsep}{NNLO$_\text{sep}$}
\newcommand{\NNLOsat}{\ensuremath{\mathrm{NNLO}_{\mathrm{sat}}}}
\newcommand{\Info}{\mathcal{H}}
\newcommand{\dobs}{\tilde{d}}
\newcommand{\Htilde}{\tilde{H}}
\newcommand{\ModelT}{\text{T}}

\newcommand{\Aaug}{\matr{A}_{\textrm{aug}}}
\newcommand{\thetavec}{\bm{\theta}}
\newcommand{\dataset}[3]{\ensuremath{{\textrm #1}#2_{(#3\%)}}}
%\newcommand{\kmax}{k_{\text{max}}}

\newcommand{\Cprime}{C$'$}

% notation for matrices
%\newcommand{\matr}[1]{\mathbf{#1}} % undergraduate algebra version
\newcommand{\matr}[1]{#1}          % pure math version
%\newcommand{\matr}[1]{\bm{#1}}     % ISO complying version

\newcommand{\transpose}[1]{{#1}^{\intercal}}
\newcommand{\trans}{\intercal}


\newcommand{\ktrue}{k^{\rm true}}
\newcommand{\atrue}{a^{\rm true}}
\newcommand{\avecmin}{\hat\avec}
\newcommand{\Nd}{N_d}

\newcommand{\chiEFT}{$\chi$EFT}
\newcommand{\chisq}{\chi^2}
\newcommand{\chisqaug}{\chisq_{\textrm aug}}
\newcommand{\avecaug}{\avec_{\textrm aug}}

\newcommand{\CHtoEKM}{CH\_to\_EKM}
\newcommand{\LamchiSB}{\Lambda_{\chi {\rm SB}}}
\newcommand{\chiPT}{\chi{\rm PT}}

% \newcommand{\Data}{\ensuremath{c_0,\ldots,c_k}}
\newcommand{\Aeps}{\ensuremath{{\rm A}_{\epsilon}}}
\newcommand{\Ceps}{\ensuremath{{\rm C}_{\epsilon}}}
\newcommand{\Aepsone}{\Aeps^{(1)}}
\newcommand{\Cepsone}{\Ceps^{(1)}}
\newcommand{\Aone}{\ensuremath{{\rm A}^{(1)}}}
\newcommand{\Bone}{\ensuremath{{\rm B}^{(1)}}}
\newcommand{\Cone}{\ensuremath{{\rm C}^{(1)}}}
\newcommand{\Af}[2]{\ensuremath{{\rm A}_{#1\text{-}#2}}}
\newcommand{\Cf}[2]{\ensuremath{{\rm C}_{#1\text{-}#2}}}
\newcommand{\Afone}[2]{\Af{#1}{#2}^{(1)}}
\newcommand{\Cfone}[2]{\Cf{#1}{#2}^{(1)}}
\newcommand{\Deltakone}{\ensuremath{\Delta_k^{(1)}}}
\newcommand{\dkp}{\ensuremath{d_k^{(p)}}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\sbarmin}{\sbar_{<}}
\newcommand{\sbarmax}{\sbar_{>}}
\newcommand{\ppercentt}{\ensuremath{\left(p\%\right)_{\rm t}}}

% \newcommand{\Xref}{\ensuremath{\mathcal{X}_{\text{ref}}}}
% \newcommand{\Xrefinput}{\ensuremath{\mathbcal{X}_{\text{ref}}}}
\newcommand{\genobsref}{\ensuremath{y_{\mathrm{ref}}}}
\newcommand{\genobsrefset}{\ensuremath{\inputvec{y}_{\mathrm{ref}}}}
\newcommand{\genobsrefinput}{\ensuremath{\inputdimvec{y}_{\mathrm{ref}}}}

\newcommand{\Mmatrix}[3]{M^{#1}_{{#2}\,{#3}}}
\newcommand{\CG}[6]{\langle {#1}\,{#2}\; {#3}\,{#4} | {#5}\,{#6} \rangle}
\newcommand{\sigmatot}{\sigma_{\text{tot}}}
\newcommand{\sigmaref}{\sigma_{\text {ref}}}
\newcommand{\epsbar}{\bar\varepsilon}


\newcommand{\ppercent}{(100*p)\%}

% Glockle Coefficients
\newcommand{\aG}{\ensuremath a_G}
\newcommand{\bG}{\ensuremath b_G}
\newcommand{\cG}{\ensuremath c_G}
\newcommand{\mG}{\ensuremath m_G}
\newcommand{\gG}{\ensuremath g_G}
\newcommand{\hG}{\ensuremath h_G}

% Phase notation
\newcommand{\phase}[3]{\ensuremath{\bar\delta^{#1 #3}_{#2}}}
\newcommand{\blattphase}[3]{\ensuremath{\delta^{#1 #3}_{#2}}}
\newcommand{\epsmix}[1]{\ensuremath{\bar\epsilon_{#1}}}
\newcommand{\blattepsmix}[1]{\ensuremath{\epsilon_{#1}}}
\newcommand{\gammix}[1]{\ensuremath{\bar\gamma_{#1}}}

% R on-shell
\newcommand{\Ron}[4]{R^{#1 #4}_{#2 #3}}


% Lab system / center of momentum system
\newcommand{\ls}{l.s.}
\newcommand{\cms}{c.m.}

\newcommand{\kf}{\ensuremath{k_{\scriptscriptstyle\textrm{F}}}}
\newcommand{\kfzero}{\ensuremath{k_{\scriptscriptstyle\textrm{F,0}}}}

\newcommand{\NEVC}{\ensuremath{N_{\rm EVC}}}


% Differential taken from Physics package
% Uses smart spacing for a nice look. Requires xparse.
% https://www.ctan.org/pkg/physics?lang=en

% First, the basics:
\def\diffd{\mathrm{d}}  % Upright differentials
% \def\diffd{d}  % Italic differentials

% Now add spacing:
% Derivatives
\DeclareDocumentCommand\differential{ o g d() }{ % Differential 'd'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
            {\diffd\IfNoValueTF{#1}{}{^{#1}}}
            {\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
        }
        {\mathinner{\diffd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
    }
\DeclareDocumentCommand\dd{}{\differential} % Shorthand for \differential


% Path Derivative:
\newcommand{\pathd}{\mathcal{D}}  % differential symbol for path integrals

% Now add relevant spacing and options
% Inspired by differential definition from `Physics' package at
% https://www.ctan.org/tex-archive/macros/latex/contrib/physics?lang=en
\DeclareDocumentCommand\pathdifferential{ o g d() }{ % Path 'D'
    % o: optional n for nth differential
    % g: optional argument for readability and to control spacing
    % d: long-form as in d(cos x)
    \IfNoValueTF{#2}{
        \IfNoValueTF{#3}
            {\pathd\IfNoValueTF{#1}{}{^{#1}}}
            {\mathinner{\pathd\IfNoValueTF{#1}{}{^{#1}}\argopen(#3\argclose)}}
        }
        {\mathinner{\pathd\IfNoValueTF{#1}{}{^{#1}}#2} \IfNoValueTF{#3}{}{(#3)}}
    }

\DeclareDocumentCommand\DD{}{\pathdifferential} % Shorthand for \pathdifferential

% Observable notation

% \newcommand{\dsigma}{\ensuremath{\frac{\partial\sigma}{\partial\Omega}}}

% \makeatletter
% \def\dsigma{\@ifstar\@@dsigmawithstar\@dsigma}
% \def\@dsigma{\frac{\dd\sigma}{\dd\Omega}}  % \dsigma for upright frac
% \def\@@dsigmawithstar{\dd\sigma/\dd\Omega} % \dsigma* for inline frac
% \makeatother

% From physics package. Optimal braces.
% \DeclareDocumentCommand\argopen{s}{\IfBooleanTF{#1}{\mathopen{}\mathclose\bgroup}{\mathopen{}\mathclose\bgroup\left}} % Special open grouping for argument of a function
% \DeclareDocumentCommand\argclose{s}{\IfBooleanTF{#1}{\egroup}{\aftergroup\egroup\right}} % Special close grouping for argument of a function

% \DeclareDocumentCommand\braces{}{{\ifnum\z@=`}\fi\@braces}
% \DeclareDocumentCommand\@braces{ s t\big t\Big t\bigg t\Bigg m m m }
% { % General braces with automatic and manual sizing
%     \IfBooleanTF{#1}
%     {\left#6\smash{#8}\right#7\vphantom{#8}}
%     {
%         \IfBooleanTF{#2}{\bigl#6{#8}\bigr#7}{
%             \IfBooleanTF{#3}{\Bigl#6{#8}\Bigr#7}{
%                 \IfBooleanTF{#4}{\biggl#6{#8}\biggr#7}{
%                     \IfBooleanTF{#5}{\Biggl#6{#8}\Biggr#7}{\left#6{#8}\right#7}
%                 }
%             }
%         }
%     }
%     \ifnum\z@=`{\fi}
% }

% \DeclareDocumentCommand\fbraces{ s t\big t\Big t\bigg t\Bigg m m m m }
% { % Function braces with automatic and manual sizing
%     #8
%     \IfBooleanTF{#1}
%     {\argopen#6\smash{#9}\argclose#7\vphantom{#9}}
%     {
%         \IfBooleanTF{#2}{\argopen*\bigl#6{#9}\argclose*\bigr#7}{
%             \IfBooleanTF{#3}{\argopen*\Bigl#6{#9}\argclose*\Bigr#7}{
%                 \IfBooleanTF{#4}{\argopen*\biggl#6{#9}\argclose*\biggr#7}{
%                     \IfBooleanTF{#5}
%                     {\argopen*\Biggl#6{#9}\argclose*\Biggr#7}
%                     {\argopen#6{#9}\argclose#7}
%                 }
%             }
%         }
%     }
% }
% \DeclareDocumentCommand\opbraces{ m g o d() }
% {
%     \IfNoValueTF{#2}
%     {
%         \IfNoValueTF{#3}
%             {
%                 \IfNoValueTF{#4}
%                 {#1}
%                 {\fbraces{\lparen}{\rparen}{#1}{#4}}
%             }
%             {
%                 \fbraces{\lbrack}{\rbrack}{#1}{#3}
%                 \IfNoValueTF{#4}{}{(#4)}
%             }
%     }
%     {
%         \fbraces{\lbrace}{\rbrace}{#1}{#2}
%         \IfNoValueTF{#3}{}{[#3]}
%         \IfNoValueTF{#4}{}{(#4)}
%     }
% }

% \let\exponential\exp \DeclareDocumentCommand\exp{}{\opbraces{\exponential}}

